Scaling Structured Inference with Randomization

Deep discrete structured models have seen considerable progress recently, but traditional inference using dynamic programming (DP) typically works with a small number of states (less than hundreds), which severely limits model capacity. At the same time, across machine learning, there is a recent trend of using randomized truncation techniques to accelerate computations involving large sums. Here, we propose a family of randomized dynamic programming (RDP) algorithms for scaling structured models to tens of thousands of latent states. Our method is widely applicable to classical DP-based inference (partition, marginal, reparameterization, entropy) and different graph structures (chains, trees, and more general hypergraphs). It is also compatible with automatic differentiation: it can be integrated with neural networks seamlessly and learned with gradient-based optimizers. Our core technique approximates the sum-product by restricting and reweighting DP on a small subset of nodes, which reduces computation by orders of magnitude. We further achieve low bias and variance via Rao-Blackwellization and importance sampling. Experiments over different graphs demonstrate the accuracy and efficiency of our approach. Furthermore, when using RDP for training a structured variational autoencoder with a scaled inference network, we achieve better test likelihood than baselines and successfully prevent posterior collapse. code at: https://github.com/FranxYao/RDP

==> 031_method_alg_viterbi.tex <==
\begin{algorithm}[tb]
  \caption{Randomized Viterbi}
  \label{alg:viterbi}
\begin{algorithmic}
  \STATE {\bfseries Input:} data $x_i$, size $m$
  \REPEAT
  \STATE Initialize $noChange = true$.
  \FOR{$i=1$ {\bfseries to} $m-1$}
  \IF{$x_i > x_{i+1}$}
  \STATE Swap $x_i$ and $x_{i+1}$
  \STATE $noChange = false$
  \ENDIF
  \ENDFOR
  \UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}

==> 031_method_proposal.tex <==
% Although all oracle proposals for RDP algorithms require full summation and are hard to get, we can exploit the unnormalized local potentials as lower-order information for proposal construction. 
% Specifically, for each node, we suggest a proposal by locally-normalizing the potentials:
% \begin{align}
%   q_t(i) = \frac{1}{2}\frac{\phi_t(i)}{\sum_{i=1}^N \phi_t(i)} + \frac{1}{2}\frac{\sum_{j=1}^N \phi_{st}(j, i)}{\sum_{i, j} \phi_{st}(j, i)} 
% \end{align}
% This is conceptually similar to a mean-field approximation to actual intermediate DP summands. 


==> 061_app_theory.tex <==
\subsection{Bias Analysis}
\label{sec:app:theory:bias}
\input{061_app_theory_bias.tex}

\subsection{Variance Analysis}
\label{sec:app:theory:variance}
\input{061_app_theory_variance.tex}

==> 061_app_theory_rb.tex <==
In this section, we show how Eq.~\ref{eq:tailsum} can be interpreted as Rao-Blackwellization. 
Fristly, Rao-Blackwellization says that a function $J$ depending on two random variables $X, Y$ has larger variance than its conditional expectation~\citep{pmlr-v33-ranganath14}: 
\begin{align}
  \hat{J}(X) &= \mathbb{E}[J(X, Y) | X] \\
  \mathbb{V}[\hat{J}(X)] &= \mathbb{V}[J(X, Y)] - \mathbb{E}[(J(X, Y) - \hat{J}(X))^2] \le \mathbb{V}[J(X, Y)] \label{eq:rb}
\end{align}
This is because $Y$ has been integrated out and the source of randomness is reduced to $X$. 

Now consider a sorted list of positive numbers $a_1, ..., a_N$, define two uniform random index:
\begin{align}
  &\delta_1 \sim \text{Uniform}(1, 2, ..., K_1) \\
  &\delta_2 \sim \text{Uniform}(K_1 + 1, ..., N)
\end{align}
and a randomized sum:
\begin{align}
  S(\delta_1, \delta_2) = K_1 a_{\delta_1} + (N - K_1) a_{\delta_2}
\end{align}
Then the conditional expectation is defined as:
\begin{align}
  \hat{S}(\delta_2) &= \mathbb{E}[S(\delta_1, \delta_2) | \delta_2] \\ 
  &= \sum_{\delta_1 = 1}^{K_1} a_{\delta_1} + (N - K_1) a_{\delta_2}
\end{align}
Using $S(\delta_1, \delta_2), \hat{S}(\delta_2)$ to substitute $J(X, Y), \hat{J}(X)$ in Eq.~\ref{eq:rb}, we get:
\begin{align}
  \mathbb{V}[\hat{S}(\delta_2)] &\le \mathbb{V}[S(\delta_1, \delta_2)]
\end{align}
Intuitively, the variance is decreased because we sample from a smaller space. 

Additionally, changing $\delta_2$ to be from a proposal distribution $\vq$ gives us importance sampling: 
\begin{align}
  \mathbb{E}_{\delta_2 \sim \text{Uniform}}[(N - K_1)a_{\delta_2}] &=  \mathbb{E}_{\delta_2 \sim \vq}[\frac{1}{q_{\delta_2}(N-K_1)}(N - K_1)a_{\delta_2}] \\ 
  &= \mathbb{E}_{\delta_2 \sim \vq}[\frac{1}{q_{\delta_2}} a_{\delta_2}]
  % \sum_{\delta_1 = 1}^{K_1} a_{\delta_1} + \sum_{\delta_2 = K_1 + 1}^N \frac{N - K_1}{N - K_1} a_{\delta_2} \\
  % &= \sum_{\delta_1 = 1}^{K_1} a_{\delta_1} + \sum_{\delta_2 = K_1 + 1}^N \frac{q_{\delta_2}}{q_{\delta_2}} a_{\delta_2} \\ 
  % &= \mathbb{E}_{\delta_2'}[\sum_{\delta_1 = 1}^{K_1} a_{\delta_1} + (N - K_1) a_{\delta_2'}]
\end{align}
where the importance weight is $\frac{1}{q_{\delta_2}(N-K_1)}$ and the $N-K_1$ term is cancelled out. 

